Learned Trimmed-Ridge Regression for Channel Estimation in Millimeter-Wave Massive MIMO

Channel estimation poses significant challenges in millimeter-wave massive multiple-input multiple-output systems, especially when the base station has fewer radio-frequency chains than antennas. To address this challenge, one promising solution exploits the beamspace channel sparsity to reconstruct full-dimensional channels from incomplete measurements. This paper presents a model-based deep learning method to reconstruct sparse, as well as approximately sparse, vectors fast and accurately. To implement this method, we propose a trimmed-ridge regression that transforms the sparse-reconstruction problem into a least-squares problem regularized by a nonconvex penalty term, and then derive an iterative solution. We then unfold the iterations into a deep network that can be implemented in online applications to realize real-time computations. To this end, an unfolded trimmed-ridge regression model is constructed using a structural configuration to reduce computational complexity and a model ensemble strategy to improve accuracy. Compared with other state-of-the-art deep learning models, the proposed learning scheme achieves better accuracy and supports higher downlink sum rates.

==> method.tex <==
\section{Gradient projection descent algorithms under DC programming framework on trimmed ridge regression for sparse reconstructions}
	In this section, we present the TRR formulation for sparse reconstruction, followed by the derivation of a single-loop iterative solution for TRR. 
	The TRR is a nonconvex optimiztion problem. We adopt the DC programming approach to solve it and derive a single-loop iterative gradient projection descent (GPD) algorithm by a special DC decomposition.
	Then, we change the step size strategy and present two GPD algorithms for TRR.
	These two GPD algorithms will be used for deep unfolding in the next section. 

\subsection{Trimmed ridge regression for sparse reconstruction}

While \eqref{MMV} is a multiple measurement vectors (MMV) problem, we treat it as multiple parallel single measurement vector (SMV) problems so that our proposed method can apply to both MMV and SMV problem. 
To this end, we use the vector $\mathbf x$ to represent uniquely the real part $\Re (\mathbf h_b)$ and the imaginary part $\Im (\mathbf h_b)$ of a beamspace channel vector. Thus, the sparse channel reconstruction can be described as the following linear system,
	\begin{IEEEeqnarray*}{lCl} \label{linear_equation}
	\mathbf y = \mathbf \Phi \mathbf x+ \mathbf n
	\IEEEyesnumber
	\end{IEEEeqnarray*} 	
	where $\mathbf y \in \mathbb{R}^{L}$, $\mathbf \Phi \in \mathbb{R}^{L \times N_{BS}}$, $\mathbf x \in \mathbb{R}^{N_{BS}}$, $\mathbf n \in  \mathbb{R}^{L}$, and $L \ll N_{BS}$. 
The under-determined linear equation \eqref{linear_equation} can be solved by the following constrained least squares optimization
	\begin{IEEEeqnarray*}{lCl} \label{SRopt}
	\min \limits_{\mathbf{x}} &&\quad  \norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2\\
	\text{s.t.} &&\quad \norm{\mathbf{x}}_0  \le K.
	\IEEEyesnumber
	\end{IEEEeqnarray*}
The $\ell_0$-constraint $\norm{\mathbf{x}}_0  \le K$ in \eqref{SRopt} results in an NP-hard optimization. We introduce the  top-$(K,2)$ norm $\norm{\mathbf x}^2_{(K,2)}$ to replace the $\ell_0$-constraint $\norm{\mathbf{x}}_0  \le K$ \cc{cite}. 
The top-$(K,2)$ norm is the sum of squares of the $K$ elements that have largest magnitudes for the vector $\mathbf x$, i.e.,
	\begin{IEEEeqnarray*}{lCl} \label{}
	\norm{\mathbf x}^2_{(K,2)} = :=  x^2_{(1)} + x^2_{(2)} + \cdots + x^2_{(K)}
	\IEEEyesnumber
	\end{IEEEeqnarray*}
where $x_{(i)}$ denotes the element whose magnitude is the $i$th-largest among the $N$ elements of the vector $\mathbf x$, i.e., $ | x_{(1)} | \ge| x_{(2)} | \ge \cdots \ge | x_{(N)} |$.
By adopting the top-$(K,2)$ norm, we have the equal relationship of $\norm{\mathbf x}^2-\norm{\mathbf x}^2_{(K,2)}=0 \leftrightarrow \norm{\mathbf{x}}_0  \le K$. Thus, we rewrite the sparse reconstruction problem \eqref{SRopt} as
	\begin{IEEEeqnarray*}{lCl} \label{SRopt_topK2}
	\min \limits_{\mathbf{x}} &&\quad  \norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2\\
	\text{s.t.} &&\quad \norm{\mathbf x}^2-\norm{\mathbf x}^2_{(K,2)}=0.
	\IEEEyesnumber
	\end{IEEEeqnarray*}
By using the Lagrange multiplier $\rho$, we transform \eqref{SRopt_topK2} into an unconstrained optimization problem 
	\begin{IEEEeqnarray*}{lCl} \label{SRopt_topK2_unconstrain}
	\min \limits_{\mathbf{x}} \quad 
	\frac{1}{2}\norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2 
	+ \rho (\norm{\mathbf x}^2_2 - \norm{\mathbf x}^2_{(K,2)})
	:=F(\mathbf x).
	\IEEEyesnumber
	\end{IEEEeqnarray*}
We name the optimization \eqref{SRopt_topK2_unconstrain} the trimmed ridge regression (TRR) since the \eqref{SRopt_topK2_unconstrain} is similar to a ridge regression, i.e., $\min \limits_{\mathbf x} \frac{1}{2}\norm{\mathbf{y}-\mathbf{\Phi}\mathbf{x}}_2^2 + \rho \norm{\mathbf x}^2_2$ but it only has a different regularizer. The novel regularizer is more favourable to obtaining accurate and sparse solution since it removes the penalties on the $K$ largest-magnitude elements of the reconstructing vector. 
	
\subsection{Solving Trimmed Ridge Regression Using Gradient Projection Descent Algorithms Under DC programming Framework}
	We will derive  a valid iterative solution for the trimmed ridge regression using the DC programming framework and the gradient projection descent method. We first write the objective in the trimmed ridge regression problem \eqref{SRopt_topK2_unconstrain} by  
 	\begin{IEEEeqnarray*}{lCl} \label{obj_k2norm}
	F(\mathbf x)
	=
	 \frac{l}{2} \norm{\mathbf x}_2^2 -  \frac{l}{2} \norm{\mathbf x}_2^2 + \frac{1}{2}\norm{\mathbf y - \mathbf {\Phi x}}_2^2  + \rho (\norm {\mathbf x}_2^2 - \norm{\mathbf x}^2_{K,2})
	\IEEEyesnumber
	\end{IEEEeqnarray*}
where $l \ge 0$ is a Lipschitz constant of the least square objective $\frac{1}{2}\norm{\mathbf y - \mathbf {A x}}_2^2$.
	Then, we perform the following DC decomposition on the objective function in \eqref{obj_k2norm}, and we obtain 
	\begin{IEEEeqnarray*}{lCl}
	\label{obj_x_dc}
	\min_\mathbf x 
	\underbrace{ \frac{l}{2} \norm{\mathbf x}_2^2 + \rho \norm {\mathbf x}_2^2}_{f(\mathbf x)} - \underbrace{ \left( \frac{l}{2} \norm{\mathbf x}_2^2- \frac{1}{2}\norm{\mathbf y - \mathbf {\Phi x}}_2^2
	 + \rho \norm{\mathbf x}^2_{K,2} \right)}_{g(\mathbf x)}
	\IEEEyesnumber
	\end{IEEEeqnarray*}
	where the functions $f(\mathbf x)$ and $g(\mathbf x)$ are convex. 
	The convexity of $g(\mathbf x)$ can be ensured by confirming the convexity of $\frac{l}{2} \norm{\mathbf x}_2^2- \frac{1}{2}\norm{\mathbf y - \mathbf {\Phi x}}_2^2$, which is shown in Appendix \cc{TODO}.
	
	
Next, we split the positive and negative parts of $\mathbf x$ by letting $\mathbf u = (\mathbf x)_+, \mathbf v = (-\mathbf x)_+$, where $(\cdot)_+$ is the positive-taking operation that retains the positive elements and sets the other elements to be zeros. More precisely, $(\mathbf x)_+$ represents for each element $x$ in vector $\mathbf x$ we take $(x)_+ = \max \{0, x\}$;  $(-\mathbf x)_+$ represents for each element $-x$ in vector $-\mathbf x$ we take $(-x)_+ = \max \{0, -x\}$.
By denoting $\mathbf{z} = [\mathbf{u}^{T}, \mathbf{v}^{T}]^{T}$, $\mathbf A = [\mathbf \Phi, -\mathbf \Phi]$ we can express \eqref{obj_x_dc} as 
	\begin{IEEEeqnarray*}{lCl} \label{obj_z_dc}
	\min_{\mathbf{z} \succeq \mathbf{0}} \quad
	\underbrace{ \frac{l}{2} \norm{\mathbf z}_2^2 + \rho \norm {\mathbf z}_2^2}_{f(\mathbf z)} - \underbrace{ \left( \frac{l}{2} \norm{\mathbf z}_2^2- \frac{1}{2}\norm{\mathbf y - \mathbf {A z}}_2^2
	 + \rho \norm{\mathbf z}^2_{K,2} \right)}_{g(\mathbf z)}
	\IEEEyesnumber
	\end{IEEEeqnarray*}
To solve \eqref{obj_z_dc}, we recall the DC programming procedure, that is, for the arbitrary $t$th iteration computing the the gradient (or subgradient) $ \partial g(\mathbf z^{t})$ and then solving the convex subproblem $\min \limits_{\mathbf{z}\succeq \mathbf{0}}  f(\mathbf z) - \mathbf z^T \partial g(\mathbf z^{t})$ to obtain $\mathbf z^{(t+1)}$. In other words, we perform the following two steps repeatedly until convergence:
	\begin{IEEEeqnarray*}{lCl} \label{dc_procedure}
	(\text{a}) \quad 
	\partial g(\mathbf z^{(t)}) 
	=  l \mathbf{z}^{(t)} - (\mathbf y - \mathbf{A} \mathbf{z}^{(t)}) + 2 \rho \mathbf{\overline{z}}^{(t)}_{K} \\	
	(\text{b}) 
	\quad \mathbf z^{(t+1)} = \arg \min \limits_{\mathbf{z} \succeq \mathbf{0}} 
	  \big\{\frac{l}{2} \norm{\mathbf z}_2^2 + \rho \norm{\mathbf z}_2^2 - \mathbf z^T \partial g(\mathbf z^{(t)})\big\}. 
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
	
The subproblem (b) in \eqref{dc_procedure} has a closed-form optimal solution. To show it, we rewrite the optimization (b) in \eqref{dc_procedure} as
	\begin{IEEEeqnarray*}{lCl} \label{prob_closed_z}
	\min\limits_{\mathbf z \succeq \mathbf{0}} && \quad
	\frac{l+2\rho}{2} \big(\norm{\mathbf z}_2^2 - \mathbf z^T \partial g(\mathbf z^{t}) \big)
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
	Next, the problem \eqref{prob_closed_z} can be expressed as
	\begin{IEEEeqnarray*}{lCl}
	\label{proj_prob_closed_z}
	\min \limits_{\mathbf z \succeq \mathbf{0}} 
	&& \quad
	\frac{l+2\rho}{2} \norm{\mathbf z - \frac{1}{l+2\rho}\partial g(\mathbf z^{t}) }_2^2
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
	The objective in \eqref{proj_prob_closed_z} is to minimize a quadratic function with respect to the vector $\mathbf z$ over the set $\mathbf z \succeq \mathbf 0$.
	We can obtain a closed-form optimal solution to \eqref{proj_prob_closed_z}, that is simply the Euclidean projection of $\frac{1}{l+2\rho} \partial g(\mathbf z^{t})$ onto the nonnegative orthant. The optimal solution to \eqref{proj_prob_closed_z} can be expressed as follows
	\begin{IEEEeqnarray*}{lCl} \label{optimal_z_closed}
	\mathbf z^* = \left( \frac{1}{l+2\rho} \partial g(\mathbf z^{t}) \right)_+.
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
	The DC programming procedure in \eqref{dc_procedure} reduces to update repeatedly the following two single-step computations until convergence:
	\begin{IEEEeqnarray*}{lCl} \label{dc_alg_closed}
	(\text{a}) 
	\quad  \partial g(\mathbf z^{t})  =  l \mathbf{z}^{t} - (\mathbf y - \mathbf{A} \mathbf{z}^{t}) + 2 \rho \mathbf{\overline{z}}^{t}_{K} \\	
	(\text{b}) 
	\quad \mathbf z^{(t+1)} 
	 = \left( \frac{1}{l+2\rho} \partial g(\mathbf z^{t}) \right)_+.
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
Next, we substitute $\partial g(\mathbf z^{t})$ in (a) into (b) of \eqref{dc_alg_closed} such that (a) and (b) can be combined to be the $t$th update for $\mathbf z^{t}$ 
	\begin{IEEEeqnarray*}{lCl}
	\label{interpret_t_update}
	\mathbf z^{(t+1)}  
	&&= \left( \frac{1}{l+2\rho} \left( l \mathbf z^{t} + 2 \rho \mathbf z^{t} - 2 \rho \mathbf z^{t} - \mathbf{A}^T (\mathbf y - \mathbf{A} \mathbf{z}^{t}) + 2 \rho \mathbf{\overline{z}}^{t}_{K} \right) \right)_+ \\
	&& = \big( \mathbf z^{t} - \frac{1}{l+2\rho} \underbrace{\left(\mathbf{A}^T (\mathbf y - \mathbf{A} \mathbf{z}^{t})+ 2 \rho \mathbf z^{t}-  2 \rho \mathbf{\overline{z}}^{t}_{K} \right)}_{\nabla F(\mathbf z^{t})} \big)_+.
	\IEEEyesnumber  
	\end{IEEEeqnarray*} 
    
    The iteration \eqref{interpret_t_update} is a valid iterative solution for TRR. Since \eqref{interpret_t_update} is derived from DC programming method, the update \eqref{interpret_t_update} shares the same global convergence as DC programming. 
    More importantly, we make a crucial interpretation that \eqref{interpret_t_update} is a GPD update for the proposed TRR optimization problem \eqref{SRopt_topK2_unconstrain}.
%    \begin{IEEEeqnarray*}{lCl}
%	\label{bcqp_closed}	
%	\min \limits_{\mathbf z \succeq  \mathbf 0} \quad 
%	\frac{1}{2}\norm{\mathbf{y}-\mathbf{A}\mathbf{z}}_2^2 
%	+ \rho (\norm{\mathbf z}^2_2 - \norm{\mathbf z}^2_{(K,2)})
%	:= F(\mathbf z).
%	\IEEEyesnumber  
%	\end{IEEEeqnarray*} 
   
   It should note that the gradient projection descent update \eqref{interpret_t_update} requires with a special step size $1/(l+2\rho)$, where $l= \lambda_{\text{max}}(\mathbf A^T \mathbf A)$ is the maximal eigenvalue of $\mathbf A^T \mathbf A$; $\rho$ is the regularization parameter. 
   The $t$th-step update of the GPD iteration can be expressed as
    \begin{IEEEeqnarray*}{lCl} \label{basic_GPD}
    \mathbf{z}^{(t+1)} &= \left(\mathbf{z}^{(t)} - \frac{1}{l+2\rho} \nabla F(\mathbf{z}^{(t)})\right)_+
     \IEEEyesnumber
    \end{IEEEeqnarray*}
    where $(\cdot)_+$ is the projection operation that projects a vector onto the nonnegative orthant \footnote{The nonnegative orthant is the generalization of the first quadrant to $n$-dimensions for $n \ge 2$.}.
    To unfold the GPD iterations of TRR, we first change the fixed step size $1/(l+2\rho)$ and design the variable step size strategy to develop more generic GPD algorithms for TRR. 

\subsection{GPD Algorithms with Variable Step-sizes for TRR}    
    \subsubsection{Monotonic BB-step-size GPD iteration (MoGPD)} 
    The $t$th-step update can be expressed as
    \begin{IEEEeqnarray*}{lCl} \label{mono_GPD}
    \mathbf{w}^{(t+1)} &= \left(\mathbf{z}^{(t)} - \alpha^{(t)} \nabla F(\mathbf{z}^{(t)})\right)_+,\\
     \mathbf{z}^{(t+1)} &= \mathbf{z}^{(t)} + \beta^{(t)} ( \mathbf{w}^{(t+1)}  -  \mathbf{z}^{(t)} ).
     \IEEEyesnumber
    \end{IEEEeqnarray*}
	where $\alpha^t > 0$ is the step size for the $t$th update; $\beta^t \in (0, 1]$ is the extrapolation parameter to prevent the step size being over large and ensure that the objective value can descent monotonically.
	We further accelerate the gradient projection iterations using Nesterov’s acceleration method as follows.
	\subsubsection{Nesterov’s accelerated GPD iteration (NaGPD)}    
	 The $t$th-step update can be expressed as
	\begin{IEEEeqnarray*}{lCl} \label{NA_GPD}
	\mathbf{w}^{(t+1)} &= \left(\mathbf{z}^{(t)} - \alpha^{(t)} \nabla F(\mathbf{z}^{(t)})\right)_+,\\
	\mathbf{z}^{(t+1)} &=  \mathbf{w}^{(t+1)}  + \beta^{(t)} ( \mathbf{w}^{(t+1)}  -   \mathbf{w}^{(t)}).
	\IEEEyesnumber
	\end{IEEEeqnarray*}
	
	In \eqref{basic_GPD}, \eqref{mono_GPD} and \eqref{NA_GPD}, $\nabla F(\mathbf{z}^{(t)})$ represents the gradient of the function $F(\cdot)$ in terms of $\mathbf{z}^{(t)}$ which is calculated by $\nabla F(\mathbf z^{(t)}) = \mathbf{A}^T (\mathbf y - \mathbf{A} \mathbf{z}^{(t)})+ 2 \rho \mathbf z^{(t)}-  2 \rho \mathbf{\overline{z}}^{(t)}_{K} $.
	 The fixed step size $\frac{1}{l+2\rho}$ in \eqref{basic_GPD} is generalized to be the variable step size $\alpha^t > 0$ in \eqref{mono_GPD} and \eqref{NA_GPD}.
	The extrapolation parameter $\beta^t \in (0, 1]$ can prevent the descent step being too large.
	
	
	We summarize the updates \eqref{mono_GPD} and \eqref{NA_GPD} for TRR into Algorithm 1 and Algorithm 2, which can be directly applied to sparse reconstructions for compressive sensing. For beamspace channel estimation, one can adopt random measurement matrices to design pilot matrix and then reconstruct channel reconstruction using Algorithm 1 or Algorithm 2 \bb{TODO:compare traditional and unfolding convergences}.
	However, we will focus on developing data-driven methods to further exploit the data-driven advantages and will unfold Algorithm 1 and Algorithm 2 to build deep compressive sensing autoencoders in the next section.
	\begin{algorithm}
	\caption{Basic gradient projection descent (BaGPD) for TRR} 
	\hspace*{\algorithmicindent} \textbf{Input:} measurements $\mathbf y$, matrix $\mathbf A$ and a small number $\epsilon$ \\
    \hspace*{\algorithmicindent} \textbf{Output:} reconstructed $\hat{\mathbf x}$ \\
    	\hspace*{\algorithmicindent} \textbf{Initialization:}  $\mathbf u^{(0)}$, $\mathbf v^{(0)}$, $\mathbf z^{(0)} \leftarrow [(\mathbf u^{(0)})^T,  (\mathbf v^{(0)})^T]^T$
	\begin{algorithmic}[1]
		\For {$t=1,2,\ldots$}
			\State $\nabla F(\mathbf z^{(t)}) \leftarrow \mathbf{A}^T (\mathbf y - \mathbf{A} \mathbf{z}^{(t)})+  \rho (\mathbf z^{(t)}-\mathbf{\overline{z}}^{(t)}_{K})$
			\State $\mathbf{z}^{(t+1)} \leftarrow \left(\mathbf{z}^{(t)} - \frac{1}{l+2\rho} \nabla F(\mathbf{z}^{(t)})\right)_+$ 
			\State Check terminate condition $\norm{\mathbf z^{(t+1)}-\mathbf z^{(t)}}_2 \le \epsilon$, return to Step 1 if not satisfied; otherwise, terminate with $\mathbf z^{(t+1)} =  [(\mathbf u^{(t+1)})^T,  (\mathbf v^{(t+1)})^T]^T$, and return $\hat{\mathbf x} = \mathbf u^{(t+1)} - \mathbf v^{(t+1)}$.
		\EndFor
	\end{algorithmic} 
\end{algorithm}

	\begin{algorithm}
	\caption{Trimmed ridge regression via monotone gradient projection descent (TRR-MoGPD)} 
	\hspace*{\algorithmicindent} \textbf{Input:} measurements $\mathbf y$, matrix $\mathbf A$ and a small number $\epsilon$ \\
    \hspace*{\algorithmicindent} \textbf{Output:} reconstructed $\hat{\mathbf x}$ \\
    	\hspace*{\algorithmicindent} \textbf{Initialization:}  $\mathbf u^{(0)}$, $\mathbf v^{(0)}$, $\mathbf z^{(0)} \leftarrow [(\mathbf u^{(0)})^T,  (\mathbf v^{(0)})^T]^T$
	\begin{algorithmic}[1]
		\For {$t=1,2,\ldots$}
			\State $\nabla F(\mathbf z^{(t)}) \leftarrow \mathbf{A}^T (\mathbf y - \mathbf{A} \mathbf{z}^{(t)})+  \rho (\mathbf z^{(t)}-\mathbf{\overline{z}}^{(t)}_{K})$
			\State $\mathbf{w}^{(t+1)}  \leftarrow \left(\mathbf{z}^{(t)} - \alpha^{(t)} \nabla F(\mathbf{z}^{(t)})\right)_+$
			\State $\mathbf{z}^{(t+1)} \leftarrow \mathbf{z}^{(t)} + \beta^{(t)} (\mathbf{w}^{(t+1)}  -  \mathbf{z}^{(t)} )$
			\State Check terminate condition $\norm{\mathbf z^{(t+1)}-\mathbf z^{(t)}}_2 \le \epsilon$, return to Step 1 if not satisfied; otherwise, terminate with $\mathbf z^{(t+1)} =  [(\mathbf u^{(t+1)})^T,  (\mathbf v^{(t+1)})^T]^T$, and return $\hat{\mathbf x} = \mathbf u^{(t+1)} - \mathbf v^{(t+1)}$.
		\EndFor
	\end{algorithmic} 
\end{algorithm}


	\begin{algorithm}
	\caption{Trimmed ridge regression via Nesterov's accelerated gradient projection descent (TRR-NaGPD)} 
	\hspace*{\algorithmicindent} \textbf{Input:} measurements $\mathbf y$, matrix $\mathbf A$ and a small number $\epsilon$ \\
    \hspace*{\algorithmicindent} \textbf{Output:} reconstructed $\hat{\mathbf x}$ \\
    	\hspace*{\algorithmicindent} \textbf{Initialization:}  $\mathbf u^{(0)}$, $\mathbf v^{(0)}$, $\mathbf z^{(0)} \leftarrow [(\mathbf u^{(0)})^T,  (\mathbf v^{(0)})^T]^T$
	\begin{algorithmic}[1]
		\For {$t=1,2,\ldots$}
			\State $\nabla F(\mathbf z^{(t)}) \leftarrow \mathbf{A}^T (\mathbf y - \mathbf{A} \mathbf{z}^{(t)})+  \rho (\mathbf z^{(t)}-\mathbf{\overline{z}}^{(t)}_{K})$
			\State $\mathbf{w}^{(t+1)} = \left(\mathbf{z}^{(t)} - \alpha^{(t)} \nabla F(\mathbf{z}^{(t)})\right)_+ $
			\State $\mathbf{z}^{(t+1)} = \mathbf{w}^{(t+1)} + \beta^{(t)} (\mathbf{w}^{(t+1)} -  \mathbf{w}^{(t)})$
			\State Check terminate condition $\norm{\mathbf z^{(t+1)}-\mathbf z^{(t)}}_2 \le \epsilon$, return to Step 1 if not satisfied; otherwise, terminate with $\mathbf z^{(t+1)} =  [(\mathbf u^{(t+1)})^T,  (\mathbf v^{(t+1)})^T]^T$, and return $\hat{\mathbf x} = \mathbf u^{(t+1)} - \mathbf v^{(t+1)}$.
		\EndFor
	\end{algorithmic} 
\end{algorithm}



\section{TRR Autoencoder by Deep Unfolding for Data-Driven Pilot Design and Channel Estimation}
	In the last section, starting from applying GPD to DC programming framework to solve the TRR optimization problem, we derived two sparse reconstruction algorithms including TRR-MoGPD and TRR-NaGPD. 
	Instead of using the proposed algorithms directly to perform iterative sparse reconstructions, we will adopt deep unfolding technique to unfold them into stacking layers of deep networks and fit the unfolded deep network as the decoder of a customized autoencoder. In another words, we treat each individual step of the iterative algorithms as a layer of decoder for the constructing autoencoder. 
 	In this section, we will design deep unfolding autoencoders based on the proposed TRR algorithms. 
 	Since the built autoencoders mimic the process of compressive sensing and sparse reconstruction, we name this method deep compressive sensing and name the built autoencoder unfolding TRR autoencoder (UTRRA).
	In the following subsections, we first present the framework of UTRRA and then present its two types of decoder structures by unfolding TRR-MoGPD or TRR-NaGPD algorithms. 
	Then, we discuss the pipeline of joint pilot design and beamspace channel estimation using the proposed UTRRA.
	
\subsection{The Structure of TRR Autoencoder (TRRAE) by Deep Unfolding}


\begin{figure}[!t]
\centering
\includegraphics[scale=0.3]{./figures/LTRRA.png}
\captionsetup{justification=centering}
\caption{The framework of TRRAE \bb{Modify: "unfolding reconstruction layers"}}
\label{gpsa_structure}
\end{figure}

	 
	The proposed deep compressive sensing autoencoder framework is shown in Fig. \ref{gpsa_structure}, consisting of a \mbox{single-layer} encoder and a \mbox{multi-layer} decoder. 
	
	\subsubsection*{Encoder}The encoder performs a linear dimension reduction $\mathbf{y} = \mathbf{\Phi} \mathbf{x}$. 
	The input sparse vector $\mathbf{x}$ is projected onto the subspace spanned by the columns of the measurement matrix $\mathbf{\Phi}$ to get the compressed measurement vector $\mathbf{y}$.
	
	The decoder plays the role of the sparse reconstruction from $\mathbf{y}$ to $\hat{\mathbf{x}}$ in a feed-forward manner. 	
	The decoder is constructed to mimic the TRR sparse reconstruction algorithms.
	To interpret the decoder, we separate it into three parts, which correspond to the initialization, forward update and output phase of the aforementioned sparse reconstruction algorithm.
	
	\emph{Initializing decoder layer ($\mathbf y$ to $\mathbf z^{(0)}$):} The first two layers can be interpreted as the initialization phase of the sparse reconstruction algorithm, that is from the input compressed measurement matrix $\mathbf{r}$ to get the initialized positive vector $\mathbf{z}^{(0)}$.
	For the first layer, instead of simply initializing $\mathbf{x}^{(0)}$ to be zero as the conventional sparse recovery strategy, we set 
    \begin{IEEEeqnarray*}{lCl}
    \mathbf{x}^{(0)}= \mathbf{\Phi}^\mathrm{T} \mathbf{r}. 
    \IEEEyesnumber
    \end{IEEEeqnarray*}
	The second layer plays the role to prepare an equivalent positive initialization vector $\mathbf{z}^{(0)}$ by separating and concatenating the positive and negative part of $\mathbf{x}^{(0)}$, that is $\mathbf{z}^{(0)}=[(\mathbf{u}^{(0)})^\mathrm{T}, (\mathbf{v}^{(0)})^\mathrm{T}]^\mathrm{T}$, where $\mathbf{u}^{(0)} = \text{ReLU}(\mathbf{x}^{(0)})$ and $\mathbf{v}^{(0)} = \text{ReLU}(-\mathbf{x}^{(0)})$.
	
	\subsubsection*{Unfolding reconstruction layers ($\mathbf{z}^{(1)}$ to $\mathbf{z}^{(L)}$)} The second part of the decoder performs a forward update from $\mathbf{z}^{(0)}$ to $\mathbf{z}^{(T)}$, which consists of $T$ \mbox{structural-identical} blocks. Each block is one-step iteration by unfolding the sparse reconstruction algorithm. In specific, we cast the update steps of the gradient projection descent or its acceleration algorithm into stacked layers of the decoder, and set the measurement matrix $\mathbf{\Phi}$ as the tied weight matrix for each layer. 
	We construct two types of structures for the unfolding reconstruction layers by unfolding the proposed TRR-MoGPD and TRR-NaGPD updates. The single layer structures of unfolding TRR-MoGPD and TRR-NaGPD updates are shown in Fig. \ref{MoGPD_decoder} and Fig. \ref{NaGPD_decoder}.
	It is worth noting that the ReLU activation function in unfolding layers are the exact replacement of the projection operations $(\cdot)_+$ in TRR-MoGPD and TRR-NaGPD updates.
	We empirically set the extrapolation parameter as $\beta^t =  \frac{t}{t+3}$. 
	
		
	%\begin{figure}[!t]
	%\centering
	%\includegraphics[scale=0.35]{./figures/BaGPD_decoder.png}
	%\captionsetup{justification=centering}
	%\caption{A single-layer decoder by unfolding BaGPD for TRR}
	%\label{BaGPD_decoder}
	%\end{figure}
	
	\begin{figure}[!t]
		\centering
		\includegraphics[scale=0.33]{./figures/MoGPD_decoder.png}
		\captionsetup{justification=centering}
		\caption{A single-layer structure of unfolding MoGPD}
		\label{MoGPD_decoder}
	\end{figure}
	
	\begin{figure}[!t]
		\centering
		\includegraphics[scale=0.35]{./figures/NaGPD_decoder.png}
		\captionsetup{justification=centering}
		\caption{A single-layer structure of unfolding NaGPD}
		\label{NaGPD_decoder}
	\end{figure}

	
	\emph{Output Layer:} The last layer is the output layer, in which we obtain the recovered sparse vector $\hat{\mathbf{h}}$ from $\mathbf{z}^{(T)}$. Specifically, with $\mathbf{z}^{(T)} = [z^{(T)}_1, ..., z^{(T)}_{2N_t}]$, we have 
	\begin{IEEEeqnarray*}{lCl}
	\hat{\mathbf{h}}=\mathbf{u}^{(T)}- \mathbf{v}^{(T)},
	\IEEEyesnumber
	\end{IEEEeqnarray*}
	where $\mathbf{u}^{(T)} = [z^{(T)}_1, ..., z^{(T)}_{N_t}]$ and $\mathbf{v}^{(T)} = [z^{(T)}_{N_{t+1}}, ..., z^{(T)}_{2N_t}]$.
	
	 \subsubsection*{Loss Function}The encoder and decoder are jointly trained together to minimize the mean squared error of reconstructions. The loss function is defined as 
	 \begin{IEEEeqnarray*}{lCl}
	 \label{loss_function}
	 \mathcal{L}(\mathbf{h}, \hat{\mathbf{h}}) = \frac{1}{n} \sum_{i=1} ^{n} \norm{\mathbf{h}-\hat{\mathbf{h}}}_2^2.
	 \IEEEyesnumber
	 \end{IEEEeqnarray*}


\subsection{Offline Training and Online Application of TRRA for Joint Data-Driven Pilot Design and Channel Estimation}
	
As shown in Fig. \ref{pipeline}, the proposed TRRA is first trained offline to acquire data-driven pilots $\mathbf \Phi$ and then implemented online to estimate the beamspace channels.

We set the measurement matrix $\mathbf \Phi$ as the weights for both encoder and multiple layers of decoder so that the measurement matrix can be optimized while training using given dataset and the optimal measurement matrix $\mathbf \Phi$ can be extracted after training the autoencoder. 

As we know, given an artificial neural network and a loss function, the loss function are minimized and the weight matrices are optimized during the training process by backpropagation. 
The backpropagation algorithm calculates the gradient of the loss function with respect to the neural network's weights, and optimizes the weight matrices using gradient descent to minimize the loss function.

To use the error back propagation to optimize the measurement matrix $\mathbf{\Phi}$, we cast the measurement matrix $\mathbf{\Phi}$ as the tied and constrained weight matrices for the feed-forward layers in decoder.
This design brings two advantages.
On one hand, we keep the measurement matrix as the tied weights so that the measurement matrix are able to be fully optimized by training with given dataset.		 
On the other hand, in the forward-update layers of decoder, we purposely constraint the weight matrix of measurement matrix $\mathbf{\Phi}$ in the computational form of \eqref{gpsr_update} and \eqref{NGPS2} to obtain fast convergence so that the the constructed neural networks can keep in small size and easy to train.

The measurement matrix $\mathbf{\Phi}$ plays important role for accurate reconstruction of beamspace channel $\mathbf{\widetilde{h}}_{b,i}$ from measurements $\mathbf{\widetilde{r}}_i$. 
Instead of exploiting the random measurement matrix, we will optimize the measurement matrix $\mathbf{\Phi}$. 
Once we obtain the optimized measurement matrix $\mathbf{\Phi}^*$, equivalently we obtain the optimized pilots by $\mathbf{S}^*=(\mathbf{U}_T \mathbf{\Phi}^*)^\mathrm{H}$.

	
\begin{figure}[!t]
\centering
\includegraphics[scale=0.35]{./figures/pipeline.png}
\captionsetup{justification=centering}
\caption{Pipeline of offline training and online application of TRRA for data-driven pilot design and beamspace channel estimation \bb{TODO maybe need to modify autoencode/decoder names and add math notations}}
\label{pipeline}
\end{figure}


